Unleashing the Power of Depth and Pose Estimation Neural Networks by Designing Compatible Endoscopic Images

Deep learning models have witnessed depth and pose estimation framework on unannotated datasets as a effective pathway to succeed in endoscopic navigation. Most current techniques are dedicated to developing more advanced neural networks to improve the accuracy. However, existing methods ignore the special properties of endoscopic images, resulting in an inability to fully unleash the power of neural networks. In this study, we conduct a detail analysis of the properties of endoscopic images and improve the compatibility of images and neural networks, to unleash the power of current neural networks. First, we introcude the Mask Image Modelling (MIM) module, which inputs partial image information instead of complete image information, allowing the network to recover global information from partial pixel information. This enhances the network' s ability to perceive global information and alleviates the phenomenon of local overfitting in convolutional neural networks due to local artifacts. Second, we propose a lightweight neural network to enhance the endoscopic images, to explicitly improve the compatibility between images and neural networks. Extensive experiments are conducted on the three public datasets and one inhouse dataset, and the proposed modules improve baselines by a large margin. Furthermore, the enhanced images we proposed, which have higher network compatibility, can serve as an effective data augmentation method and they are able to extract more stable feature points in traditional feature point matching tasks and achieve outstanding performance.

==> paragraphs/limitation.tex <==
\section{Limitation}

\textcolor{blue}{As shown in Section 4.1, our proposed EVP significantly outperforms the previous state-of-the-art visual prompting method, and is even stronger than linear probing. However, with non-clip models, our simple one-to-one matching strategy does not yet achieve competitive results to linear probing.
This motivates us that there is still plenty of room for improvement
(e.g., by exploring more sophisticated one-to-multiple or even multiple-to-multiple matching strategies) in the future.}



